Pruned Landmark Labeling Meets Vertex Centric Computation: A Surprisingly Happy Marriage!

In this paper, we study how the Pruned Landmark Labeling (PPL) algorithm can be parallelized in a scalable fashion, producing the same results as the sequential algorithm. More specifically, we parallelize using a Vertex-Centric (VC) computational model on a modern SIMD powered multicore architecture. We design a new VC-PLL algorithm that resolves the apparent mismatch between the inherent sequential dependence of the PLL algorithm and the Vertex- Centric (VC) computing model. Furthermore, we introduce a novel batch execution model for VC computation and the BVC-PLL algorithm to reduce the computational inefficiency in VC-PLL. Quite surprisingly, the theoretical analysis reveals that under a reasonable assumption, BVC-PLL has lower computational and memory access costs than PLL and indicates it may run faster than PLL as a sequential algorithm. We also demonstrate how BVC-PLL algorithm can be extended to handle directed graphs and weighted graphs and how it can utilize the hierarchical parallelism on a modern parallel computing architecture. Extensive experiments on real-world graphs not only show the sequential BVC-PLL can run more than two times faster than the original PLL, but also demonstrates its parallel efficiency and scalability.

==> figures/BVCPLL.tex <==
\begin{algorithm}[H]
%\small
\scriptsize
\caption{VC-PLL for $G=(V,E)$ with Order $\pi$}
\label{alg:VertexCentricPLL_push}
\begin{algorithmic}[1]
\STATE $\forall v \in V, L (v)=\delta L(v) \gets \{(v, 0)\}, C(v) \gets \emptyset$
\WHILE{$\delta L \ne \emptyset$} 
\FORALL{$v \in V \wedge \delta L(v) \neq \emptyset$}
    \FORALL{$u \in N(v)$: $N(v)$ is $v$'s neighbor set} 
         \STATE Send all $(h \in \delta L(v): d(v,h)+1)$ to $C(u)$ where $\mathcal{O}(h) > \mathcal{O}(u)$ \AND $h \notin L(u)$ \label{alg:VertexCentricPLL_push:line:7}
    \ENDFOR % each v's neighbors
\ENDFOR % each v in V
\FORALL {$u \in V \wedge C(u) \neq \emptyset$}
    \STATE $\delta L(u) \leftarrow \emptyset$
	\FORALL {$(h: d(u,h) \in C(u)$}
		 \label{alg:VertexCentricPLL_push:line:15}
			\STATE Add $(h: d(u,h))$ to  $\delta L(u)$ if $d(u,h) < \min_{z \in L(u) \cap L(h)} d(h,z)+d(z,u)$
% 						\IF {$d(u,h) < \min_{z \in L(u) \cap L(h)} d(h,z)+d(z,u)$}
% 			   \STATE Add $(h: d(u,h))$ to  $\delta L(u)$
% 			\ENDIF
	\ENDFOR
	\STATE Add $\delta L(u)$ to $L(u)$; $C(u) \gets \emptyset$ 
\ENDFOR
\ENDWHILE
\end{algorithmic}
\end{algorithm}
